Parental Guidance: Efficient Lifelong Learning through Evolutionary Distillation

Developing robotic agents that can perform well in diverse environments while showing a variety of behaviors is a key challenge in AI and robotics. Traditional reinforcement learning (RL) methods often create agents that specialize in narrow tasks, limiting their adaptability and diversity. To overcome this, we propose a preliminary, evolution-inspired framework that includes a reproduction module, similar to natural species reproduction, balancing diversity and specialization. By integrating RL, imitation learning (IL), and a coevolutionary agent-terrain curriculum, our system evolves agents continuously through complex tasks. This approach promotes adaptability, inheritance of useful traits, and continual learning. Agents not only refine inherited skills but also surpass their predecessors. Our initial experiments show that this method improves exploration efficiency and supports open-ended learning, offering a scalable solution where sparse reward coupled with diverse terrain environments induces a multi-task setting.

==> 10_thanks.tex <==
\thanks{$^{*}$ All three authors contributed equally.}
\thanks{$^{1}$Paul G. Allen School of Computer Science and Engineering, University of Washington 
         \texttt{\small \{adityavk, rosario, bhou, siddh\}@cs.washington.edu}}%
\thanks{$^{2}$Aurora Innovation Inc. \texttt{\small sanjiban.choudhury@gmail.com}}%
\thanks{This work was (partially) funded by the National Science Foundation IIS (\#2007011), National Science Foundation DMS (\#1839371), the Office of Naval Research, US Army Research Laboratory CCDC, Amazon, and Honda Research Institute USA.}% <-this % stops a space


==> algorithms/00_cool_alg.tex <==
%------------------------------------------%
% Algorithm E4: EvolutionScheduler
%------------------------------------------%

% 

% \begin{algorithm}[t]
% \SetAlgoLined
% \caption{\texttt{EvolutionScheduler}}
% \label{alg:evolution_scheduler}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \Input{initial\_population, graph\_population, DAG graph}
% \Output{Job Information}

% Initialize population: $\mathcal{P} \gets$ initial\_population \\
% Initialize Directed Acyclic Graph (DAG) $\mathcal{G}$ \\
% \While{awaiting request \texttt{get\_next\_job}}{

%     species\_to\_evaluate $\gets \{\}$ \\
    
%     \ForEach{species $s \in \mathcal{P}$}{
%         \If{species\_status(s) == alive \textbf{and} evaluation\_status(s) == false}{
%             species\_to\_evaluate.append(s)
%         }
%     }
    
%     \eIf{len(species\_to\_evaluate) $>$ 0}{
%         evaluation\_species $\gets$ \texttt{random\_choice}(species\_to\_evaluate) \\
%         species\_id, species\_env\_cfg, species\_model $\gets$ \texttt{get\_species\_data}(evaluation\_species) \\
%         \Return{
%             \{"job\_type": "eval", \\
%             "species\_id": species\_id, \\
%             "species\_env\_cfg": species\_env\_cfg, \\
%             "species\_model": species\_model\}
%         }
%     }{
%         new\_species\_id $\gets$ \texttt{graph\_population} + 1 \\
        
%         \If{graph\_population $<$ initial\_population}{
%             \Return{
%                 \{"job\_type": "train", \\
%                 "species\_id": new\_species\_id\}
%             }
%         }{
%             living\_species $\gets$ \texttt{select\_species}(\texttt{status} == alive) \\
%             ancestors $\gets$ \texttt{fertilization\_criterion}(living\_species) \\
%             ancestors $\gets$ \texttt{random\_choice}(ancestors, 2) \\
%             ancestor\_ids, ancestors\_env\_cfg, ancestors\_models $\gets$ \texttt{ancestors\_data}(ancestors) \\
%             \Return{
%                 \{"job\_type": "eval", \\
%                 "species\_id": new\_species\_id, \\
%                 "ancestor\_ids": ancestor\_ids, \\
%                 "ancestor\_models": ancestors\_models, \\
%                 "ancestors\_env\_cfg": ancestors\_env\_cfg\}
%             }
%         }
%     }
% }

% \While{awaiting request \texttt{complete\_job}}{
%     job\_type $\gets$ request.data["job\_type"] \\
%     species\_id $\gets$ request.data["species\_id"] \\
%     \texttt{update\_progress\_status}(job\_type, species\_id)
% }
% \end{algorithm}


% %------------------------------------------%
% % Algorithm: Training with Mutation and Reproduction
% %------------------------------------------%

% \begin{algorithm}[t]
% \SetAlgoLined
% \caption{\texttt{Species Trainer}}
% \label{alg:M}

% job\_type, metadata = get\_next\_job() \newline
% Is\_offspring = False \newline


% \If{job\_type == "train"}{

%     \If{"ancestor\_ids" \textbf{in} metadata}{
%         \# Reproduction process: train with behavioral cloning (BC) objective \\
%         ancestor\_models, ancestor\_env\_cfgs = metadata["ancestor\_models"], metadata["ancestor\_env\_cfgs"] \\
        
%         \# Load ancestor models \\
%         ancestor\_models = \texttt{torch.load}(ancestor\_models) \\
        
%         \# Perform genetic breeding to create hybrid environment configuration \\
%         hybrid\_env\_cfg = \texttt{genetic\_breed}(ancestor\_env\_cfgs) \\
        
%         env = hybrid\_env\_cfg \\
%         Is\_offspring = True \\
%     }
%     \Else{
%         \# Initialize with default configuration for mutation-only process \\
%         default\_cfg = \texttt{initialize\_default\_cfg} \\
%         env = default\_cfg \\
%     }

%     \# Apply genetic mutation to the environment configuration \\
%     env = \texttt{genetic\_mutate}(env) \\
    
%     \# Initialize the environment \\
%     env = \texttt{gym.make}(env) \\

%     \If{Is\_offspring}{
%         \# Training with ancestor models (RL with behavior cloning loss) \\
%         \texttt{learn\_with\_ancestors}(env)
%     }
%     \Else{
%         \# Standard training \\
%         \texttt{learn}(env)
%     }
% }
% \end{algorithm}

\begin{algorithm}[b]
\SetAlgoLined
\caption{Method Overview}
\label{alg:learn_with_expert}
\KwIn{Number of iterations $N$, Expert policies $\{\pi_E^t\}$, Student policies $\pi_{S}$ }
Initialize $\pi_{S}$, $\lambda$; \Comment{$\lambda$ is bc weight decay rate}\;
\For{i $=1$ \KwTo $N$}{
    \For{step $=1$ \KwTo num\_steps\_per\_env}{
        Use policy $\pi_{S}$ to sample rollouts $\mathcal D:=\{(obs, a_s, reward)\}$ \;
        \For{each terrain $t$}{
            Obtain expert $\pi_E^t$ actions mean $\mu_E^t$ and std $\sigma_E^t$ from $\pi_E^t$\;
        }
        % Update policy storage with new $\{(obs, reward)\}$\;
    }
    \For{each $d$ in $\mathcal D$}{
        % Compute action log probabilities and values\;
        Compute surrogate loss $\mathcal{L}_{\text{surrogate}}$\ and value loss $\mathcal{L}_V$, and total BC loss base on Eqn.~\ref{eq:bcloss}:
        
        Compute total loss $\mathcal{L}$ and update $\pi_{S}$ based on Eqn.~\ref{eq:distill}
        % \[
        % \mathcal{L} = \lambda^i \cdot \mathcal{L}_{\text{BC}} + (1 - \lambda^i) \cdot (\mathcal{L}_{\text{surrogate}} - c \cdot \text{entropy}) + \beta \mathcal{L}_V
        % \]
    }
}
\end{algorithm}


==> figures/00_long_fig_with_caption_breakdown.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/guild_mechanism.pdf}
\caption{
\textbf{(a)}
Initial solution.
\textbf{(b)}
\guild{} selects a beacon and induces Local Subsets (green), which do not cover the narrow passage.
\textbf{(c)}
The planner does not find a shorter path to the goal, so the Informed Set is unchanged.
However, \guild{} leverages the improved cost-to-come in the search tree to update the Local Subsets.
The start-beacon set shrinks to further focus sampling,
and the remaining slack between the beacon's and goal's cost-to-comes is used to \emph{expand} the beacon-target set.
The Local Subsets now cover the narrow passage,
focusing sampling within the Informed Set to quickly converge to
\textbf{(d)}
the optimal solution.
}
\label{fig:ideal_scenario}
\vspace{2\baselineskip}
\end{figure*}

==> figures/01_long_subfig_env.tex <==
\begin{figure*}[!ht]
\setlength{\fboxrule}{1pt}
\setlength{\fboxsep}{0pt}
\newlength{\envwidth}
\setlength{\envwidth}{0.18\linewidth}
\centering
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/env_images/forest_hard.png}}
  \caption{\forestenv}
  \label{fig:forestenv}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/env_images/two_wall_forest_hard.png}}
  \caption{\twowallforestenv}
  \label{fig:twowallforestenv}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/env_images/L_forest.png}}
  \caption{\lforestenv}
  \label{fig:lforestenv}
\end{subfigure}\hspace{2em}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/env_images/maze.png}}
  \caption{\carenv}
  \label{fig:carenv}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/env_images/v4.png}}
  \caption{\herbenv}
  \label{fig:herbenv}
\end{subfigure}
\caption{
Evaluation environments.
% \forestenv, \twowallforestenv, and \lforestenv are $\R^2$ planning problems.
% \carenv is an $SE(2)$ planning problem, and
% \herbenv is an $\R^7$ planning problem.
}
\label{fig:envs}
\setlength{\fboxrule}{0.2pt}
\setlength{\fboxsep}{3pt}
\vspace{-1\baselineskip}
\end{figure*}

==> figures/02_compact_fig_with_subfig_env.tex <==
\begin{figure}[!t]
\centering
\setlength{\fboxrule}{1pt}
\setlength{\fboxsep}{0pt}
\newlength{\heatmapwidth}
\setlength{\heatmapwidth}{0.22\linewidth}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_uniform_1.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_uniform_12.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_uniform_15.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_uniform_24.png}}

\medskip

\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_informed_1.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_informed_20.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_informed_30.png}}
\fbox{\includegraphics[width=\heatmapwidth]{figs/heatmap_informed_38.png}}
\caption{
Snapshots of the sample heatmap for \uniformguild (top) and IS (bottom) on the \forestenv environment.
% at \bhnote{A, B, C samples} and convergence.
Regions that have been sampled more densely are more red.
\uniformguild densifies around the optimal path more quickly than IS.
}
\label{fig:filmstrip}
\setlength{\fboxrule}{0.2pt}
\setlength{\fboxsep}{3pt}
\vspace{-1\baselineskip}
\end{figure}

==> macros/math_operators.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\argmaxprob}[1]{\underset{#1}{\argmax}}
\newcommand{\argminprob}[1]{\underset{#1}{\argmin}}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\suchthat}{\;\; \mbox{s.t.} \;\;}
\newcommand{\abs}[1]{\left|#1 \right|}
\newcommand{\pair}[2]{\left( #1, #2\right)}
\newcommand{\set}[1]{\left\lbrace #1\right\rbrace}
\newcommand{\seq}[2]{\left(#1_{1}, #1_{2}, \ldots, #1_{#2}\right)}
\newcommand{\seqset}[2]{\left\lbrace#1_{1}, #1_{2}, \ldots, #1_{#2}\right\rbrace}
\newcommand{\setst}[2]{\left\lbrace #1\;\middle|\;#2\right\rbrace}
\newcommand{\setInsert}[0]{\xleftarrow{\scriptscriptstyle +}}
\newcommand{\setRemove}[0]{\xleftarrow{\scriptscriptstyle -}}
\newcommand{\Ind}[0]{\mathbb{I}} % Indicator Function
\newcommand{\expect}[2]{\mathbb{E}_{#1}\left[#2\right]}

==> tables/00_small_table.tex <==
\begin{table}[t]
\caption{Model performance on both \emph{Development} and \emph{Test} {\bf Robot Pairs}.}
\centering
\begin{tabular}{l c c r r}
	\toprule
    & \multicolumn{2}{c}{\bf Model ($M$)} & \multicolumn{2}{c}{\bf Detection Correct $\uparrow$} \\
	&  Ego &  Object & \multicolumn{1}{c}{\IN{}} & \multicolumn{1}{c}{\ON{}} \\
	\midrule
	\multirow{5}{*}{\rotatebox{90}{\emph{Dev} Fold}}
	& \checkmark &          & $.69\pm.08$ & $.55\pm.11$ \\
	% &            & pre        &  &  \\
	& \checkmark & \checkmark & $.70\pm.09$ & $.59\pm.07$ \\
	& \checkmark & pre        & $.73\pm.09$ & $.62\pm.07$ \\
	\cmidrule{2-5}
	& \multicolumn{2}{l}{Baseline (MC)} & $.32\pm.00$ & $.36\pm.00$ \\
	& \multicolumn{2}{l}{Baseline (Rand)} & $.49\pm.06$ & $.50\pm.06$ \\
	\midrule
	\multirow{5}{*}{\rotatebox{90}{\emph{Test} Fold}} 
	& \checkmark &            & $.77\pm.05$ & $.53\pm.10$ \\
	% &            & pre        &  &  \\
	& \checkmark & \checkmark & $.74\pm.07$ & $.59\pm.08$ \\
	& \checkmark & pre        & $.77\pm.05$ & $.59\pm.06$ \\
	\cmidrule{2-5}
    & \multicolumn{2}{l}{Baseline (MC)} & $.20\pm.00$ & $.32\pm.00$ \\
    & \multicolumn{2}{l}{Baseline (Rand)} & $.52\pm.05$ & $.51\pm.07$ \\
	\bottomrule
	\multicolumn{5}{p{5cm}}{\checkmark indicates signal was included, while ``pre" indicates models with object features pretrained from {\bf All Pairs} data.}
\end{tabular}
\label{tab:results}
\end{table}

==> tables/01_large_table_with_images.tex <==
\begin{table*}[ht!]
    \caption{
    Egocentric \ego{} model and augmented \egoPobj{} model predictions. We display only the post-manipulation frame for $R_\Delta$.
    }
    \centering
    \footnotesize
    \begin{tabular}{@{}c>{\columncolor[gray]{0.9}}ccp{16em}>{\columncolor[gray]{0.9}}ccp{9em}@{}}
    \toprule
    \bf Egocentric
    \hfill $\Rightarrow$ & Pred & 
    \multicolumn{2}{l}{\bf Egocentric + Pretrained Object} \hfill $\Rightarrow$ & Pred & Truth & Reason\\
    \midrule
    \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/063-f_marbles+065-a_cups+rgb.jpeg}} 
    & \multirow{2}{*}{\cellcolor{red!25}\xmark In} 
        & \raisebox{-0.8\height}{\includegraphics[width=0.14\linewidth]{figs/063-f_marbles-stack.jpeg}} & \emph{small black sphere}, \emph{round black item}, \emph{small marble}, \emph{the blue object}, \emph{round object}, \emph{tiny object}, \emph{tiny dot}, \emph{blue round object}, \emph{little ball} & \multirow{2}{*}{\cellcolor{blue!25} \cmark In} 
        & \multirow{2}{*}{\cmark In} & \multirow{2}{9em}{With egocentric vision alone, it is difficult to see the small marble.
        After adding object data, the model classifies the \emph{tiny} marble \IN{} the \emph{cup} container.} \\
    \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/063-f_marbles+065-a_cups+d.jpeg}}
    & \cellcolor{red!25}
        & \raisebox{-.8\height}{\includegraphics[width=0.14\linewidth]{figs/065-a_cups-stack.jpeg}} & \emph{red cup}, \emph{orange cup}, \emph{small round container}, \emph{object that holds drinks}, \emph{small red cup}, \emph{red cup}, \emph{medium size cup without handles}, \emph{red plastic thing}, \emph{red cylinder} & \cellcolor{blue!25} & &  \\
    \midrule
       \raisebox{-.9\height}{\includegraphics[width=0.15\linewidth]{figs/044_flat_screwdriver+065-a_cups+rgb.jpeg}} 
       & \multirow{2}{*}{\cellcolor{red!25} \xmark In} 
        & \raisebox{-.9\height}{\includegraphics[width=0.14\linewidth]{figs/044_flat_screwdriver-stack.jpeg}} & \emph{screwdriver}, \emph{thing with the fat handle and metal prong on the end}, \emph{tool used for tightening screws}, \emph{screw driver with long tip}, \emph{screwdriver}, \emph{plastic handle screw driver}, \emph{non phillips screw driver}, \emph{tool}, \emph{black screwdriver} & \multirow{2}{*}{\cellcolor{blue!25} \cmark In} 
        & \multirow{2}{*}{\cmark In} & \multirow{2}{9em}{The reflective screwdriver and its tag spill over the edge of the cup, creating a misleading egocentric depth scan.
        After adding object data, the model classifies the \emph{screwdriver} as being \IN{} the \emph{cup} container.} \\
    \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/044_flat_screwdriver+065-a_cups+d.jpeg}} 
    & \cellcolor{red!25}
        & \raisebox{-.8\height}{\includegraphics[width=0.14\linewidth]{figs/065-a_cups-stack.jpeg}} & \emph{red cup}, \emph{orange cup}, \emph{small round container}, \emph{object that holds drinks}, \emph{small red cup}, \emph{red cup}, \emph{medium size cup without handles}, \emph{red plastic thing}, \emph{red cylinder} & \cellcolor{blue!25} &  &  \\
    \midrule
       \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/073-g_lego_duplo+065-a_cups+rgb.jpeg}} 
       & \multirow{2}{*}{\cellcolor{red!25} \xmark On} 
        & \raisebox{-.8\height}{\includegraphics[width=0.14\linewidth]{figs/073-g_lego_duplo-stack.jpeg}} & \emph{blue thing}, \emph{blue plastic rectangle}, \emph{blue plastic block}, \emph{blue cube}, \emph{lego piece}, \emph{blue plastic thing}, \emph{blue block}, \emph{small square block}, \emph{little blue block} & \multirow{2}{*}{\cellcolor{blue!25} \cmark On} 
        & \multirow{2}{*}{\cmark On} & \multirow{2}{9em}{The block rests partially nested in the cup, exhibiting a rare hybrid of both \ON{} modalities (resting on top versus nested inside).
        After adding object data, the \emph{small block} is classified as resting \ON{} the \emph{cup} container.} \\
    \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/073-g_lego_duplo+065-a_cups+d.jpeg}} 
    & \cellcolor{red!25}
        & \raisebox{-.8\height}{\includegraphics[width=0.14\linewidth]{figs/065-a_cups-stack.jpeg}} & \emph{red cup}, \emph{orange cup}, \emph{small round container}, \emph{object that holds drinks}, \emph{small red cup}, \emph{red cup}, \emph{medium size cup without handles}, \emph{red plastic thing}, \emph{red cylinder} & \cellcolor{blue!25} & &  \\
    \midrule
    \raisebox{-.9\height}{\includegraphics[width=0.15\linewidth]{figs/011_banana+010_potted_meat_can+rgb.jpeg}} 
    & \multirow{2}{*}{ \cellcolor{blue!25} \xmark On} 
        & \raisebox{-0.9\height}{\includegraphics[width=0.14\linewidth]{figs/011_banana-stack.jpeg}} & \emph{yellow thing}, \emph{long yellow item}, \emph{soft yellow thing}, \emph{yellow curved cylinder}, \emph{yellow fruit}, \emph{the object that is mostly yellow with slight green at one of the tips}, \emph{yellow long fruit}, \emph{yellow banana}, \emph{banana} & \multirow{2}{*}{\cellcolor{red!25} \cmark On} 
        & \multirow{2}{*}{\xmark On} & \multirow{2}{9em}{Given object data predictions pretrained on crowdsourced labels, the model predicts that \emph{fruit} is balanced \ON{} the \emph{can}, consistent with human ability.
        In reality, the robot manipulator lacks the dexterity to reliably balance the banana.} \\
    \raisebox{-.8\height}{\includegraphics[width=0.15\linewidth]{figs/011_banana+010_potted_meat_can+d.jpeg}}
    & \cellcolor{blue!25}
        & \raisebox{-.8\height}{\includegraphics[width=0.14\linewidth]{figs/010_potted_meat_can-stack.jpeg}} & \emph{spam}, \emph{canned meat}, \emph{metal can}, \emph{can of spam}, \emph{aluminum cube}, \emph{blue and gold cube}, \emph{rectangular can}, \emph{square}, \emph{glass circle} & \cellcolor{red!25} & &  \\
    \bottomrule
    \end{tabular}
    \label{tab:cherry_lemon}
\end{table*}
